Hyperbolic Equations for Vacuum Gravity Using Special Orthonormal Frames

By adopting Nester's higher dimensional special orthonormal frames (HSOF) the tetrad equations for vacuum gravity are put into first order symmetric hyperbolic (FOSH) form with constant coefficients, independent of any time slicing or coordinate specialization.

==> fig1.tex <==
{\nopagenumbers
\magnification=\magstep0
\hoffset = -0.1 in
\hsize=10.6 true in
\settabs 4\columns
\font\bigbold = cmbx10 scaled \magstep1
\font\bigbo = cmbx10 scaled \magstep2
\font\smallfive = cmr8
\font\smallitalic = cmti8
$$
\left(\matrix
{
D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{2}&D_{1}&
-D_{1}&\cdot&D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{2}&\cdot&\cdot\cr
\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{2}&\cdot&-D_{3}&
D_{3}&-D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{3}&\cdot\cr
\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{1}&D_{3}&\cdot&
\cdot&D_{1}&-D_{3}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{1}\cr
\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&D_{1}&-D_{3}&\cdot&
\cdot&-D_{1}&D_{3}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{3}&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&D_{2}&-D_{1}&
D_{1}&\cdot&-D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{1}&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&-D_{2}&\cdot&D_{3}&
-D_{3}&D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{2}\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{1}&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{2}&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{3}\cr
\cdot&D_{2}&-D_{1}&D_{1}&\cdot&-D_{2}&\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot\cr
-D_{2}&\cdot&D_{3}&-D_{3}&D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot&D_{4}&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{3}&\cdot&\cdot&\cdot&\cdot\cr
D_{1}&-D_{3}&\cdot&\cdot&-D_{1}&D_{3}&\cdot&\cdot&\cdot&\cdot&\cdot&D_{4}&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{1}&\cdot&\cdot&\cdot\cr
-D_{1}&D_{3}&\cdot&\cdot&D_{1}&-D_{3}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&
D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{3}&\cdot&\cdot&\cdot&\cdot&\cdot\cr
\cdot&-D_{2}&D_{1}&-D_{1}&\cdot&D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&
\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{1}&\cdot&\cdot&\cdot&\cdot\cr
D_{2}&\cdot&-D_{3}&D_{3}&-D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&
\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{2}&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&-D_{1}&\cdot&\cdot&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&-D_{2}&\cdot&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&D_{4}&\cdot&\cdot&-D_{3}&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{2}&\cdot&\cdot&
-D_{3}&\cdot&\cdot&-D_{1}&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&-D_{3}&D_{2}\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{3}&\cdot&
\cdot&-D_{1}&\cdot&\cdot&-D_{2}&\cdot&\cdot&D_{4}&\cdot&D_{3}&\cdot&-D_{1}\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{1}&
\cdot&\cdot&-D_{2}&\cdot&\cdot&-D_{3}&\cdot&\cdot&D_{4}&-D_{2}&D_{1}&\cdot\cr
D_{2}&\cdot&\cdot&D_{3}&\cdot&\cdot&D_{1}&\cdot&\cdot&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{3}&-D_{2}&D_{4}&\cdot&\cdot\cr
\cdot&D_{3}&\cdot&\cdot&D_{1}&\cdot&\cdot&D_{2}&\cdot&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{3}&\cdot&D_{1}&\cdot&D_{4}&\cdot\cr
\cdot&\cdot&D_{1}&\cdot&\cdot&D_{2}&\cdot&\cdot&D_{3}&\cdot&\cdot&\cdot&
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{2}&-D_{1}&\cdot&\cdot&\cdot&D_{4}\cr
}
\right)
\left(\matrix
{
 N_{12}\cr
 N_{23}\cr
 N_{31}\cr
 N_{13}\cr
 N_{21}\cr
 N_{32}\cr
 N_{11}\cr
 N_{22}\cr
 N_{33}\cr
 K_{12}\cr
 K_{23}\cr
 K_{31}\cr 
 K_{13}\cr
 K_{21}\cr
 K_{32}\cr
 K_{11}\cr
 K_{22}\cr
 K_{33}\cr
 a_{1}\cr
 a_{2}\cr
 a_{3}\cr
 \omega_{1}\cr
 \omega_{2}\cr
 \omega_{3}\cr
}
\right)
$$
\vskip 1in
Figure 1: The FOSH operator shown acting on the connection coefficients.
Dot indicates zero.
\vfill\eject
\end



==> fig23.tex <==
\nopagenumbers
\magnification=\magstep0
\hoffset=.21 true in
\hsize=6 true in
\settabs 4\columns
\font\bigbold = cmbx10 scaled \magstep1
\font\bigbo = cmbx10 scaled \magstep2
\font\smallfive = cmr10
\font\smallfive = cmr10
\font\smallitalic = cmti10
$$
\left(\matrix
{
D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{3}&\cdot&D_{2}\cr
\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{3}&-D_{1}&\cdot\cr
\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{1}&-D_{2}\cr
\cdot&\cdot&\cdot&2D_{4}&\cdot&\cdot&D_{3}&-D_{3}&\cdot&\cdot&D_{2}&-D_{1}\cr
\cdot&\cdot&\cdot&\cdot&2D_{4}&\cdot&\cdot&D_{1}&-D_{1}&-D_{2}&\cdot&D_{3}\cr
\cdot&\cdot&\cdot&\cdot&\cdot&2D_{4}&-D_{2}&\cdot&D_{2}&D_{1}&-D_{3}&\cdot\cr
\cdot&\cdot&\cdot&D_{3}&\cdot&-D_{2}&D_{4}&\cdot&\cdot&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&-D_{3}&D_{1}&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&-D_{1}&D_{2}&\cdot&\cdot&D_{4}&\cdot&\cdot&\cdot\cr
-D_{3}&D_{3}&\cdot&\cdot&-D_{2}&D_{1}&\cdot&\cdot&\cdot&2D_{4}&\cdot&\cdot\cr
\cdot&-D_{1}&D_{1}&D_{2}&\cdot&-D_{3}&\cdot&\cdot&\cdot&\cdot&2D_{4}&\cdot\cr
D_{2}&\cdot&-D_{2}&-D_{1}&D_{3}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&2D_{4}\cr
}
\right)
\left(\matrix
{
 A_{11}\cr
 A_{22}\cr
 A_{33}\cr
 A_{12}\cr
 A_{23}\cr
 A_{31}\cr
 B_{11}\cr
 B_{22}\cr
 B_{33}\cr
 B_{12}\cr
 B_{23}\cr
 B_{31}\cr 
}
\right)
$$
\vskip 1in
Figure 2: The FOSH operator shown acting on the Weyl components.
\vskip 2 truecm
$$
\left(\matrix
{
D_{3}&-D_{1}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot\cr
-D_{1}&D_{3}&-D_{2}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot\cr
\cdot&-D_{2}&D_{3}&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&D_{3}&-D_{1}\cdot&\cdot&\cdot&\cdot&\cr
\cdot&\cdot&\cdot&-D_{1}&D_{3}&-D_{2}&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&-D_{2}&D_{3}&\cdot&\cdot&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&D_{3}&-D_{1}&\cdot\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{1}&D_{3}&-D_{2}\cr
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&-D_{2}&D_{3}\cr
}
\right)
\left(\matrix
{
 N_{11}\cr
 N_{31}\cr
 N_{21}\cr
 N_{12}\cr
 N_{32}\cr
 N_{22}\cr
 N_{13}\cr
 N_{33}\cr
 N_{23}\cr
}
\right)
$$
\vskip 1in
Figure 3: The FOSH operator in 2+1 gravity shown acting on the 
components $N_{ab}$.
\vfill\eject
\end

